Surf at MEDIQA 2019: Improving Performance of Natural Language Inference in the Clinical Domain by Adopting Pre-trained Language Model

While deep learning techniques have shown promising results in many natural language processing (NLP) tasks, it has not been widely applied to the clinical domain. The lack of large datasets and the pervasive use of domain-specific language (i.e. abbreviations and acronyms) in the clinical domain causes slower progress in NLP tasks than that of the general NLP tasks. To fill this gap, we employ word/subword-level based models that adopt large-scale data-driven methods such as pre-trained language models and transfer learning in analyzing text for the clinical domain. Empirical results demonstrate the superiority of the proposed methods by achieving 90.6% accuracy in medical domain natural language inference task. Furthermore, we inspect the independent strengths of the proposed approaches in quantitative and qualitative manners. This analysis will help researchers to select necessary components in building models for the medical domain.

==> rsc/fig_example.tex <==
\begin{figure*}[t]
\small
\centering
\includegraphics[width=2.0\columnwidth]{rsc/example.png}
\caption{
Examples from the development set of MedNLI.
}
\label{fig:example}
\end{figure*}

==> rsc/table_data_ex_performance.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{L{0.43\columnwidth}C{0.20\columnwidth}C{0.20\columnwidth}C{0.20\columnwidth}C{0.20\columnwidth}C{0.20\columnwidth}C{0.20\columnwidth}}

\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{BioBERT}} &\multicolumn{2}{c}{\textbf{BioBERT (transferred)}}  \\
\cmidrule{2-7}
%\textbf{Dataset} & \textbf{BERT} & \textbf{BioBERT} & \textbf{BioBERT(transferred)}\\
& dev & test &  dev &   test & dev & test \\

\midrule
MedNLI & 79.56 &77.49 & 82.15 &79.04 & 83.51 & 82.63 \\

%\hline
MedNLI (expanded) & 79.13 & 77.07 & 83.87&78.76 & 82.72&81.19 \\

\bottomrule
\end{tabular}
\caption{The results of data expansion.
}
\label{table:data_ex_performance}
\end{table*}

==> rsc/table_tl_performance.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{L{0.70\columnwidth}C{0.25\columnwidth}C{0.25\columnwidth}C{0.25\columnwidth}C{0.25\columnwidth}}

\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{BioBERT}} \\
\cmidrule{2-5}
 & dev & test &  dev &   test \\
\midrule
MedNLI & 79.56 & 77.49 & 82.15 & 79.04 \\
MNLI & \textbf{83.52} & - & 81.23 & - \\
SNLI & \textbf{90.39} & - & \textbf{89.10} & - \\

\midrule
MNLI $\to$ MedNLI & 80.14 & \textbf{78.62} & 82.72 & 80.80 \\
SNLI $\to$ MedNLI & 80.28 & \textbf{78.19} & 83.29 & \textbf{81.29} \\

\midrule
MNLI $\to$ SNLI $\to$ MedNLI &  80.43 & 78.12 & 83.29 & 80.30 \\
SNLI $\to$ MNLI $\to$ MedNLI &  81.72 & 77.98 &  \textbf{83.51} & \textbf{82.63} \\

\bottomrule
\end{tabular}
\caption{The results of transfer learning on 7 different combinations of MedNLI, SNLI, and MNLI (top-2 scores marked as bold).
}
\label{table:transfer_learning}
\end{table*}




% \begin{table*}[t]
% \centering
% \begin{tabular}{L{0.70\columnwidth}C{0.55\columnwidth}C{0.55\columnwidth}}

% \hline
% \textbf{Dataset} & \textbf{BERT} & \textbf{BioBERT}\\
% &Dev/Test &Dev/Test \\

% \hline
% MedNLI & 79.56/77.49 & 82.15/79.04 \\
% MNLI & 83.52/- & 81.23/- \\
% SNLI & 90.39/- & 89.10/- \\

% \hline
% MNLI $\to$ MedNLI & 80.14/78.62 & 82.72/80.80 \\
% SNLI $\to$ MedNLI & 80.28/78.19 & 83.29/81.29 \\

% \hline
% MNLI $\to$ SNLI $\to$ MedNLI &  80.43/78.12 & 83.29/80.30 \\
% SNLI $\to$ MNLI $\to$ MedNLI &  81.72/77.98 &  83.51/82.63 \\

% \hline
% \end{tabular}
% \caption{The results of transfer learning on 7 different combinations of MedNLI, SNLI, and MNLI.
% }
% \label{table:transfer_learning}
% \end{table*}
